Generalized Veto Core and a Practical Voting Rule with Optimal Metric Distortion

We revisit the recent breakthrough result of Gkatzelis et al. on (single-winner) metric voting, which showed that the optimal distortion of 3 can be achieved by a mechanism called Plurality Matching. The rule picks an arbitrary candidate for whom a certain candidate-specific bipartite graph contains a perfect matching, and thus, it is not neutral (i.e, symmetric with respect to candidates). Subsequently, a much simpler rule called Plurality Veto was shown to achieve distortion 3 as well. This rule only constructs such a matching implicitly but the winner depends on the order that voters are processed, and thus, it is not anonymous (i.e., symmetric with respect to voters). We provide an intuitive interpretation of this matching by generalizing the classical notion of the (proportional) veto core in social choice theory. This interpretation opens up a number of immediate consequences. Previous methods for electing a candidate from the veto core can be interpreted simply as matching algorithms. Different election methods realize different matchings, in turn leading to different sets of candidates as winners. For a broad generalization of the veto core, we show that the generalized veto core is equal to the set of candidates who can emerge as winners under a natural class of matching algorithms reminiscent of Serial Dictatorship. Extending these matching algorithms into continuous time, we obtain a highly practical voting rule with optimal distortion 3, which is also intuitive and easy to explain: Each candidate starts off with public support equal to his plurality score. From time 0 to 1, every voter continuously brings down, at rate 1, the support of her bottom choice among not-yet-eliminated candidates. A candidate is eliminated if he is opposed by a voter after his support reaches 0. On top of being anonymous and neutral, this rule satisfies many other axioms desirable in practice.

==> sec/convexity.tex <==

For any fixed $\pq$-matching $\mvec$, we showed that the set of candidates $W(\mvec)$ admitting $\mvec$ is always convex in \cref{sec:convex} (for any consistent metric space where convexity is well-defined).
Therefore, the~winners tied at $\mvec$ are in a sense ``cohesive''.
However, the $\pq$-veto core is the union of all the $W(\mvec)$, and as such cannot be directly inferred to be convex. 


which would imply that all possible winners of $\sequentialrule$ (not only tied outcomes) exhibit a form of cohesiveness.
\citet{PluralityVeto} conjectured that the plurality veto core is always convex, though due to tie breaking issues (now resolved in \cref{sec:ties}) the question was phrased only for the special case of the peer selection setting.

%To gain further insight on the structure of the plurality veto core, \citet{PluralityVeto} considered the \emph{Peer Selection} setting, 
in which the set of voters is the same as the set of candidates.
In~this setting, each candidate has a plurality score of 1 since each voter ranks herself first, 
and thus, the~plurality veto core equals the proportional veto core.

\citet{PluralityVeto} conjectured that, in this specific setting, the plurality (or equivalently, proportional) veto core is convex for any consistent metric space (where convexity is well-defined), with convexity defined as a subset of candidates $A \subseteq C$ having no point in $C \setminus A$ lying within the interior of the convex hull of $A$ (as in \cref{prop:convexity}).


\citet{PluralityVeto} conjectured particularly for this setting that the plurality (or equivalently, proportional) veto core is convex in this setting for every consistent space (for which convexity is defined).
As in \cref{prop:convexity}, we say that a subset of candidates $A \subseteq C$ is convex if the interior of the convex hull of $A$ contains no point from $C \ A$. 
\begin{example} \label{ex:convexity}
	There are three voters $V = \SET{1, 2, 3}$ and six candidates $C = \SET{a_1, a_2, a_3, b_1, b_2, b_3}$.  
	The~rankings are as follows: 
	\begin{itemize}
		\item $a_1 \succ_1 b_1 \succ_1 a_2 \succ_1 b_2 \succ_1 b_3 \succ_1 a_3$
		\item $a_2 \succ_2 b_3 \succ_2 a_1 \succ_2 b_2 \succ_2 b_1 \succ_2 a_3$
		\item $a_3 \succ_3 b_2 \succ_3 b_1 \succ_3 b_3 \succ_3 a_1 \succ_3 a_2$
	\end{itemize}
	Observe that $b_1$ and $b_3$ respectively admit the plurality matchings $\SET{(1, a_2), (2, a_3), (3, a_1)}$ and $\SET{(1, a_3), (2, a_1), (3, a_2)}$, while $b_2$ does not admit any plurality matching, as voters $1$ and $2$ can be only matched to $a_3$ but $\plu(a_3) = 1$. 
	Thus, $b_1$ and $b_3$ are in the plurality veto core while $b_2$ is not.
	In~\cref{fig:convexity}, we illustrate a 2-dimensional $\ell_1$-normed space consistent with these rankings where $b_2$ is a convex combination of $b_1$ and $b_3$, specifically $b_2 = \frac{b_1 + b_3}{2}$.
	This example disproves the conjecture that the plurality veto core is always convex in general. 
\end{example}

\begin{figure}[h]
	\includegraphics[scale=0.25]{fig/convexity}	
	\caption{A consistent embedding of the election in \cref{ex:convexity} into a 2-dimensional $\ell_1$-normed space such that the plurality veto core is non-convex.}
	\label{fig:convexity}
\end{figure}



